Lessons Learned Report: Super-Resolution for Detection Tasks in Engineering Problem-Solving

We describe the lessons learned from targeting agricultural detection problem-solving, when subject to low resolution input maps, by means of Machine Learning-based super-resolution approaches. The underlying domain is the so-called agro-detection class of problems, and the specific objective is to learn a complementary ensemble of sporadic input maps. While super-resolution algorithms are branded with the capacity to enhance various attractive features in generic photography, we argue that they must meet certain requirements, and more importantly, that their outcome does not necessarily guarantee an improvement in engineering detection problem-solving (unlike so-called aesthetics/artistic super-resolution in ImageNet-like datasets). By presenting specific data-driven case studies, we outline a set of limitations and recommendations for deploying super-resolution algorithms for agro-detection problems. Another conclusion states that super-resolution algorithms can be used for learning missing spectral channels, and that their usage may result in some desired side-effects such as channels' synchronization.

==> WP.tex <==
\subsection{Work-packages}
The planned research in the proposed project is organized by means of work-packages, as listed below: 
% \begin{table}[h!]
%     \centering
%     \begin{tabular}{l l}
%          (B-1) Organization & (W6) Experimental Preparations: Sys-I \\
%          (B-2) Documentation & (W7) Sensing and Data Acquisition: Sys-I \\
%          (B-3) Literature Survey & (W8) Classification Problem-Solving: Sys-I \\
%          (W1) Compilation of synthetic model problems %\label{w1} 
%          & (W9) Experimental Planning: Sys-II \\
%          (W2) Selection and adaptation of suitable DNNs & (W10) Sensing and Data Acquisition: Sys-II \\
%          (W3) Heuristic design and tuning for Approach (A-1)
%          & (W11) Classification Problem-Solving: Sys-II \\
%          (W4) Heuristic design and tuning for Approach (A-2)
%          & (W12) Analyses \\
%          (W5) Resolution Impact & (W13) Guidelines and Algorithms
%     \end{tabular}
%     \caption{Listing the proposed work-packages.\label{tab:WP}}
% \end{table}

% \michal{I suggest to organize the work-packages in a different way.
% Following I present two ways.
% \begin{table}[h!]
%     \centering
%     \begin{tabular}{l}
%          (B1) Organization \\
%          (B2) Documentation \\
%          (B3) Literature Survey \\
%          (B4) Conference / Workshop \\
%          (W1) Compilation of synthetic model problems \\
%          (W2) Selection and adaptation of suitable DNNs  \\
%          (W3)/(W4) Heuristic design and tuning for Approach (A-1)/(A-2), respectively\\
%          (W5) Resolution Impact \\
%          (W6)/(W7) Experimental Preparations: Sys-I/Sys-II, respectively \\
%          (W8)/(W9) Sensing and Data Acquisition: Sys-I/Sys-II, respectively \\
%          (W10)/(W11) Classification Problem-Solving: Sys-I /Sys-II, respectively \\
%          (W12) Analyses \\
%          (W13) Guidelines and Algorithms
%     \end{tabular}
%     \caption{Listing the proposed work-packages.\label{tab:WP-V2}}
% \end{table}
%\michal{If we use the following suggestion, then I think it would be better to change also the notations of the approaches and the systems to be A1,A2, (instead of A-1,A-2) and S1,S2 (instead of Sys-I, Sys-II)}
\begin{table}[h!]
    \centering
    \begin{tabular}{l}
         (B1) Organization \\
         (B2) Documentation \\
         (B3) Conference / Workshop \\
         (B4) Literature survey \\
                  \newline \\
         (W1) Compilation of synthetic model problems \\
         (W2) Selection and adaptation of suitable DNNs  \\
         (W3) Heuristic design and tuning for approaches \{A1,~A2\}\\
         (W4) Resolution impact \\
         (W5) Experimental preparations for \{S1,~S2\} \\
         (W6) Sensing and data acquisition per \{S1,~S2\} \\
         (W7) Classification problem-solving \\
         (W8) Analyses \\
         (W9) Guidelines and Algorithms
    \end{tabular}
    \caption{Listing the proposed work-packages.\label{tab:WP-V1}}
\end{table}

Next, we elaborate on the work-packages that concern the primary research work of this proposal. 
Work-packages with administrative nature or straightforward activities, such as ``Organization'' or ``Documentation'' (packages B1 to B4), which set the basis for the proposed project, are not described here due to space limitations.
\begin{itemize}
    % \item[\textbf{W\ref{w1} Development of comparison metrics}] Appropriate performance metrics for ML classifiers are to be devised. Adhering to recent 
    \item[\textbf{(W1)}] \textbf{Compilation of synthetic model problems.} In order to assess our algorithms prior to field deployment, appropriate classification model problems will be synthetically generated for preliminary testing. The goal is to construct a simulator of an equivalent ML problem, which will serve as a testbed for the proposed approaches in parallel to the field sensing experiments. This will be accomplished, e.g., by artificially marking visual cues on aerial imagery and by setting it in increasing resolutions to simulate scheduled versus on-demand sensing.
    \item[\textbf{(W2)}] \textbf{Selection and adaptation of suitable DNNs.}
    DNNs are chosen as the targeted classifiers due to their capacity to treat the aforementioned ML challenges. The current package will select and adapt specific DNNs for the PA classification problem. It will capitalize on state-of-the-art CNNs (e.g., ResNet \cite{main}{He_2016_CVPR}).
    \item[\textbf{(W3)}] \textbf{Heuristic design and tuning for approaches \{A1,~A2\}. } This package deals with the realization and tuning of the algorithms employed in the project. Upon implementation, the algorithms will be deployed on the noise-free model problems (obtained in (W1)). Furthermore, their internal parameters and configurations will be fine-tuned on those problems using appropriate methodologies (e.g., SMAC \cite{main}{SMAC}).
    \item[\textbf{(W4)}] \textbf{Impact of resolution.} This work-package aims at investigating the resolution factor within the maps provided by the scheduled sensors, and its impact on the %capacity 
    ability of the proposed approaches to obtain the learning goal.
    \item[\textbf{(W5)}] \textbf{Experimental preparations for systems \{S1,~S2\}. } Prior to any sensing campaign, the actual environment (agricultural field) and the sensors have to be prepared or constructed for the experiments. 
    This work-package should start early and will have to be split into two parts, as per experimental system \{S1,~S2\}.
    %Sensing platform:
    %\rafi{I don't understnad what "applications" this is referring to. I also don't understand what are the 2 "Systems \{I,~II\} "}.
    \item[\textbf{(W6)}] \textbf{Sensing and data acquisition for systems \{S1,~S2\}. } \\
    %\td{TODO: experimental details }\\
    \textbf{S1}: RGB scans of DJI Phantom 4 Advanced multirotor unmanned aerial vehicle (UAV) and thermal scans of a DJI Matrice 600 pro UAV equipped with FLIR A655sc radiometric thermal camera will be conducted in various agricultural fields that use lateral move and pivot irrigation. Satellite images of these fields at the same dates as the UAV campaigns will be obtained, corrected and analyzed. Vegetation indices will be created for the obtained imagery in order to depict irrigation heterogeneity. \\
    \textbf{S2}: A detection system based on very high spatial resolution thermal, visible light and NIR infra-red images will be developed using UAVs, on plots that will undergo intentional inoculation, and / or naturally infected plots. Vegetation indices in the visible-NIR-SWIR spectrum (e.g. GRVI, NDVI, GNDVI, TGI, SAVI, EVI) will be used in order to examine the heterogeneity of plant vitality and for the detection of infected areas. We will examine the differences between thermal sensing and RGB-NIR sensing in detection time and intensity. In addition, we will use satellite imaging: Sentinel-2, PlanetScope, RapidEye, Ven$\mu$s (at 3-10 meters spatial resolution, average daily return time) and we will check the various satellites’ detection ability of infected areas. The state of plant health and heterogeneity will be compared between UAV and the satellite imagery via the suggested vegetation indices. Spatial analysis of the spread of the disease as a function of place and time will be carried out on a wide range of photographic findings. Because soil borne diseases are less affected by wind dispersal, we expect the spread patterns of the disease to be regular (asymmetric spread without "jumps"). We will test the rate of infection and spread of disease to neighboring plants, dynamics of disease size, disease, expansion and natural barriers to propagation.
    \item[\textbf{(W7)}] \textbf{Classification problem-solving .}  
    This work-package is concerned with the actual application of the proposed ML heuristics, which were developed in (W3), to the data obtained in (W6).
    That is, the devised algorithms will be deployed and run on the actual data. Success and failure would assist in iteratively refining the heuristics in (W3) -- coupling \textit{de factor} those two work-packages.
    \item[\textbf{(W8)}] \textbf{Comprehensive empirical investigation and analysis.} 
    The empirical results of (W7) will be analyzed in this work-package, encompassing a rigorous statistical comparison of the competing and combined approaches. 
    Standard ML classification metrics will be used to empirically evaluate each algorithmic approach, namely, Precision, Recall and the F1 index. 
    Additionally, following recent developments in the ML community, we plan to conduct statistical tests by means of Bayesian Inference \cite{main}{ML-Bayes_JMLR2017}, to verify the significance of differences in algorithmic performance.

    %Moreover, certain results from each system have to be analyzed with respect to the merit for that application. %\rafi{does this mean that toward the end of the project (last year?) we would expect to run the system in real-time, meaning that we would analyze in real-time some satellite imagery and based on that analysis send a UAV if the AI recommends it? That this to me overly ambitious given the project time frame and all the unexpected problems that are sure to crop up}
    \item[\textbf{(W9)}] \textbf{Algorithmic recommendations and guidelines formulation.} 
    The final goal and one of the outcomes of the proposed research is to provide specific guidelines on the suitability of all the proposed approaches \{A1,~A2\}, such that an answer regarding the \textit{most suitable approach} per a class of problems can be given to the practitioner. From an algorithmic perspective, we will formulate rules-of-thumb to design and launch a robust heuristic for a given task.
\end{itemize}



==> figures.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIGURES Section
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\pagebreak
\setlength\fboxsep{2.5pt}
\setlength\fboxrule{0.5pt}
\subsection{Figures}
\begin{figure}[h!]
\centering
\fbox{\includegraphics[width=0.96\linewidth]{./images/fig1.png}}
%\fbox{\epsfig{file=./images/EQS.eps, width=.9\columnwidth}}
\caption{GRVI images of the cotton field in Hagoshrim with dates indicated next to each image. GRVI values decrease from green to yellow to red.\label{fig:1}}
\end{figure}
%
\vspace*{2cm}
%
\begin{figure}[h!]
\centering
\fbox{\includegraphics[width=0.96\linewidth]{./images/fig2.png}}
    \caption{Thermal (right of pair) and corresponding GRVI images (left of pair) of the cotton field in Hagoshrim with dates indicated next to each image. Thermal images: red indicating hotter temperatures, blue colder. GRVI values decrease from green to yellow to red.\label{fig:2}}
\end{figure}
%
%%%
%
\begin{figure}[h!]
    \centering
 \fbox{\includegraphics[width=0.96\linewidth]{./images/fig3.png}}
    \caption{NDVI, GNDVI, and GRVI vegetation indices based on Venus imagery of 27/6/2018 (top) and 12/08/2018 (bottom) and the corresponding UAV GRVI image of the cotton field at 26/6/2018 and 12/08/2018, respectively.\label{fig:3}}
\end{figure}
%
\begin{figure}[h!]
    \centering
 \fbox{\includegraphics[width=0.96\linewidth]{./images/fig4.png}}
    \caption{NDVI, GNDVI, and GRVI vegetation indices based on a Sentinel-2 imagery of the cotton field in Hagoshrim test site from 20/06/2018 and the corresponding UAV GRVI Image from 17/06/2018.\label{fig:4}}
\end{figure} 
 %
\begin{figure}[h!]
    \centering
  \fbox{\includegraphics[width=0.96\linewidth]{./images/fig5.png}}
    \caption{Comparison between human inspected number of dead plants (left) and UAV borne image analysis of crop cover ratio in B77 groundnut species with 0, 100, 200 concentrations of Top-star pesticide application.\label{fig:5}}
\end{figure} 

\newlength{\mylength}
\setlength{\mylength}{\footskip}   % Saving footskip into mylength
\clearpage
\setlength{\footskip}{2.9cm}
\begin{table}[h!]
\small
   \begin{adjustbox}{center}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \hline 
    
    \makecell{ \textbf{Satellite/} \\ \textbf{sensor}} &	\makecell{\textbf{\#}\\\textbf{band}} &	\textbf{Bands} \textbf{($\mu$m)}&	\textbf{Indexes/uses} &	\makecell{\textbf{Revisit}\\ \textbf{time} \\ \textbf{(days)}} &	
    \makecell{\textbf{Spatial} \\ \textbf{resolution} \\\textbf{(m)}}	&  \makecell{\textbf{Avail-}\\\textbf{ability}} &	\textbf{Cost} &	\textbf{Owner} \\ 
    \hline
    
    Landsat-8	& 11	& 
  \makecell{0.433-0.453, \\0.450-0.515\\
0.525-0.600,\\ 0.630-0.680\\
0.845-0.885,\\ 1.56-1.66\\
2.10-2.30, \\0.50-0.68, \\1.36-1.39, \\ 10.3-11.3,\\ 11.5-12.5 } & \makecell{	NDVI \\and the like,\\ thermal,\\ Coastal /\\ Aerosol} &	16 & \makecell{	30\\ (b1-b6, b7), \\ 15 \\(pan) \\
100\\ (thermal) } &	
\makecell{ +Since \\ 1972}	 & Free	 &\makecell{ USGS/\\NASA}
 \\ 
 \hline
 
 Sentinel-2 &	13 &	\makecell{https://en.\\wikipedia.org/\\wiki/\\Sentinel-2} &
 \makecell{Agriculture, \\environment, \\aerosol, \\cloud,\\ water vapor} &	\makecell{2 \\satellites \\ -- 5 days} &	\makecell{10\\ -- RGB,\\ NIR \\20-RE,\\ SWIR,\\ 60} &	\makecell{Since\\ 2015}	& Free	& ESA
\\
\hline

Ven$\mu$s &	12	& \makecell{420, 443, \\490, 555, \\620, 620,\\ 667, 702,\\ 742, 782,\\ 865, 910} &
\makecell{Agriculture,\\ environment,\\ aerosol,\\ cloud,\\ water vapor,\\ ecosystem\\ functioning}	& 2 days &	
\makecell{5.3 
(3m \\ low orbit)} &\makecell{Since\\ 2018} &	\makecell{Free\\ (for \\research\\ purposes)} &	\makecell{ISA\\ (Israel \\space\\ agency)\\ \& ESA} \\
\hline

\makecell{MODIS -- \\Moderate-\\resolution \\ Imaging\\ Spectro-\\radiometer} & 36 & \makecell{0.4-14.4\\
https://en.\\wikipedia.\\org/wiki/\\Moderate-\\resolution\_\\imaging\_\\spectro\\radiometer}
& \makecell{Clouds,\\ aerosols,\\ photosynthetic \\activity\\ (land \\and marine),\\ land \\surface \\ changes}
& 1-2	&  \makecell{250 \\(red,\\ NIR)\\
500 \\(blue,\\ green, \\SWIR)\\
1000 \\(all \\ the\\ rest)} & \makecell{	Since \\1999}
& &\makecell{NASA --\\ Onboard \\the \\Terra \\and \\ Aqua\\ satellites}\\
\hline

\makecell{Planet-\\Scope\\ (Dove)} &	4	& 
\makecell{(nm)\\Red:\\ 610-700\\
Green:\\ 500-590\\
Blue:\\ 420-530\\
NIR:\\ 770-900}
& \makecell{Agriculture,\\ environment}	
& \makecell{daily\\CubeSat\\ -- \\constellation\\ of 88 nano-\\satellites }
& \makecell{3.7-4.9	\\ Commercial}
& \makecell{Since \\ 2013}
& \makecell{Free \\basic \\account \\ for \\academia}	
&\makecell{Planet \\ Labs} \\
\hline

\makecell{Rapid-\\Eye} &	
5	
& \makecell{(nm)\\Blue:\\440-510\\
Green:\\520-590\\
Red:\\ 630-685\\
Red Edge:\\ 690-730\\
Near IR:\\760-850}
& \makecell{Agriculture,\\ environment}
& \makecell{5 satellites\\ covering\\ 5 million\\ km2/day}
& 5	
& \makecell{Commercial \\Since \\ 2008}
& \makecell{Free \\basic \\account \\ for \\academia}	
&\makecell{Rapid-\\Eye\\ AG\\Planet \\ Labs} \\
\hline

    \end{tabular}
    \end{adjustbox}
    \caption{Technical information on satellites that are planned to be used in the proposed project.\label{tab:satellites}}
\end{table}

\clearpage
\setlength{\footskip}{\mylength}

